The Performance Analysis of Generalized Margin Maximizer (GMM) on Separable Data

Logistic models are commonly used for binary classification tasks. The success of such models has often been attributed to their connection to maximum-likelihood estimators. It has been shown that gradient descent algorithm, when applied on the logistic loss, converges to the max-margin classifier (a.k.a. hard-margin SVM). The performance of the max-margin classifier has been recently analyzed. Inspired by these results, in this paper, we present and study a more general setting, where the underlying parameters of the logistic model possess certain structures (sparse, block-sparse, low-rank, etc.) and introduce a more general framework (which is referred to as "Generalized Margin Maximizer", GMM). While classical max-margin classifiers minimize the $2$-norm of the parameter vector subject to linearly separating the data, GMM minimizes any arbitrary convex function of the parameter vector. We provide a precise analysis of the performance of GMM via the solution of a system of nonlinear equations. We also provide a detailed study for three special cases: ($1$) $\ell_2$-GMM that is the max-margin classifier, ($2$) $\ell_1$-GMM which encourages sparsity, and ($3$) $\ell_{\infty}$-GMM which is often used when the parameter vector has binary entries. Our theoretical results are validated by extensive simulation results across a range of parameter values, problem instances, and model structures.

==> MD.tex <==
\section{Finding GMM via Iterative Optimization Algorithms}
In this section, we present an iterative optimization algorithm to find the generalized margin maximizer(GMM).  More specifically, we show that when $\psi(\cdot)$ is absolutely scalable, the direction of the mirror descent iterates (with properly-tuned step size) converge to GMM. The mirror descent algorithm~\cite{nemirovsky1983problem} is a generalization of the gradient descent which is well-defined for any strongly convex, and differentiable potential $\psi(\cdot)$. \\
For our training dataset, $\mathcal D=\{(\x_i,y_i)\}_{i=1}^n$, we define the empirical loss function $\mathcal L$ as,
\begin{equation}
    \mathcal L(\mathbf w) = \sum_{i=1}^n\ell(y_i\w^T\x_i),
\end{equation}
where $\ell:\R\rightarrow \R$ is the logistic loss function defined as, $\ell(t) = \log(\frac{1}{1+e^{-t}})$. For an intialization $\w_0\in \R^p$, let $\{\w_t\}_{t\geq 0}$, be the sequence of mirror-descent iterates defined as,
\begin{equation}
    \nabla \psi(\w_{t+1}) - \nabla \psi(\w_t) = -\eta \nabla \mathcal L(\w_t).
\end{equation}
Note that the assumption on strong convexity of $\psi(\cdot)$, makes the mapping $\nabla\psi(\cdot)$ invertible. The following theorem states the convergence behavior of mirror descent iterates.
\begin{theorem}
Let $\psi:\R^d\rightarrow \R$ be an $\alpha$-strongly convex function\footnote{A function $f: \mathbb R^d\rightarrow \mathbb R$ is $m$-strongly convex if it satisfies the following,$$\big(\nabla f(\mathbf x) - \nabla f(\mathbf y)\big)^T(\mathbf x-\mathbf y)\geq m{||\mathbf x- \mathbf y||}_2^2~,~~\forall \mathbf x, \mathbf y \in \mathbb R^d.$$}. Assume $\mathcal D$ is a separable dataset and $\eta<\frac{2\alpha}{\sigma_{\max}^2(\mathbf X)}$, where $\mathbf X:=[\x_1,\x_2,\ldots,\x_n]\in \R^{p\times n}$. Then, we have,
\begin{equation}
    \lnorm{\frac{\w_t}{\lnorm{\w_t}}-\frac{\hat\w}{\lnorm{\hat\w}}}\rightarrow 0~,~\text{ as } t\rightarrow +\infty,
\end{equation}
where $\hat \w$ is the GMM classifier, that is solution of the optimization program~\eqref{eq:opt_main}.
\end{theorem}
We defer the proof of this result to the supplementary material. The main ideas behind the proof are borrowed from~\cite{soudry2018implicit}. We also provide some discussions on the convergence rate of the mirrror descent algorithm.

